Model-Independent Measurement of the e+e- -> HZ Cross Section at a Future e+e- Linear Collider using Hadronic Z Decays

A future e+e- collider, such as the ILC or CLIC, would allow the Higgs sector to be probed with a precision significantly beyond that achievable at the High-Luminosity LHC. A central part of the Higgs programme at an e+e- collider is the model-independent determination of the absolute Higgs couplings to fermions and to gauge bosons. Here the measurement of the e+e-->HZ Higgsstrahlung cross section, using the recoil mass technique, sets the absolute scale for all Higgs coupling measurements. Previous studies have considered e+e- ->ZH with Z->l+l-, where l = electron or muon. In this paper it is shown for the first time that a near model-independent recoil mass technique can be extended to the hadronic decays of the Z boson. Because the branching ratio for Z->qq is approximately ten times greater than for Z->l+l-, this method is statistically more powerful than using the leptonic decays. For an integrated luminosity of 500 fb-1 at a centre-of-mass energy of 350 GeV at CLIC, the e+e-->HZ cross section can be measured to 1.8 % using the hadronic recoil mass technique. A similar precision is found for the ILC operating at 350 GeV. The centre-of-mass dependence of this measurement technique is discussed, arguing for the initial operation of a future linear collider at just above the top-pair production threshold.

==> packages-epjc.tex <==
%\usepackage{titlepage}


\RequirePackage[T1]{fontenc}
\RequirePackage{graphicx}
\RequirePackage{mathptmx}      % use Times fonts if available on your TeX system
\RequirePackage{flushend}
\RequirePackage{feynmp}
\RequirePackage[numbers,sort&compress]{natbib}
\RequirePackage{heppennames2}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue,linkcolor=blue]{hyperref}

%\usepackage{bm}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{tocloft}
%\usepackage{texnames}
%\usepackage[T1]{fontenc}
%\pagestyle{plain}
%\usepackage{color}

%\usepackage[square,numbers,sort]{natbib}
%\usepackage{url}

%\usepackage{draftwatermark}
%\SetWatermarkFontSize{1.8cm}

%\usepackage{units}
\usepackage{booktabs}
%\usepackage{subfig}
%\usepackage{graphicx}
\usepackage{feynmp}
\DeclareGraphicsRule{*}{mps}{*}{}


%For tables
\usepackage{multirow}

%%For title layout
%\usepackage{textpos} % for placement of logo 
%\usepackage{relsize} 

%%Font treatment
%\usepackage{mathptmx}
%\usepackage[scaled=.90]{helvet}
%\usepackage{courier}
%\usepackage[T1]{fontenc} %font enconding
%\usepackage[latin9]{inputenc} %input encoding


%%Layout spacing

% align left the itemize and enumerate lists, and reduce space
%\usepackage{enumitem}
%\setlist{noitemsep}
%\setlist[itemize]{leftmargin=*, topsep=-2pt, partopsep=0pt, itemsep=2pt}
%\setlist[enumerate]{leftmargin=*, topsep=0pt, partopsep=0pt, itemsep=0pt}

% no paragraph indentation
\setlength{\parindent}{0pt}
\setlength{\parskip}{1.3ex} % less space between paragraphs

